Learning Translation Invariance in CNNs

When seeing a new object, humans can immediately recognize it across different retinal locations: we say that the internal object representation is invariant to translation. It is commonly believed that Convolutional Neural Networks (CNNs) are architecturally invariant to translation thanks to the convolution and/or pooling operations they are endowed with. In fact, several works have found that these networks systematically fail to recognise new objects on untrained locations. In this work we show how, even though CNNs are not 'architecturally invariant' to translation, they can indeed 'learn' to be invariant to translation. We verified that this can be achieved by pretraining on ImageNet, and we found that it is also possible with much simpler datasets in which the items are fully translated across the input canvas. We investigated how this pretraining affected the internal network representations, finding that the invariance was almost always acquired, even though it was some times disrupted by further training due to catastrophic forgetting/interference. These experiments show how pretraining a network on an environment with the right 'latent' characteristics (a more naturalistic environment) can result in the network learning deep perceptual rules which would dramatically improve subsequent generalization.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> other_text.tex <==

ROTATION INVARIANCE (EQUIVARIANCE?)
In order to achieve invariance to rotation, several architectural changes have been tried:
\citep{Li2017RotationNetwork}  resorted to a novel convolutional operation in order to achieve rotation invariance (stacked rotated feature maps.\citep{Marcos2016LearningClassification} tied the weights of groups of filters to rotated version of the canonical filters in the group. \citep{Gens2014DeepNetworks}, \citep{Cohen2016GroupNetworks}, and \citep{Chidester} ** NOT WORKING  used a generalization of convolution to exploit symmetry groups to describe  object transformation and show that their model can high accuracy on transformed datasets. Scattering Network \citep{Bruna2012InvariantNetworks} uses a wavelet decomposition approach for translation and rotation invariance. \citep{}* CITATION NOT PRESENT* uses crop, rotation and concatenation of input images to achieve rotation invariance

SCALE INVARIANCE
Evn though the pooling operator should support a certain degree of scale invariance, **IS THART RIGHT?  CNN do not appear to deal, in practice, with scale invariance well \citep{Gong2014Multi-scaleFeatures}, \citep{Chen2017EccentricityVision} \citep{Han2020b} and the classic solution is to include more filters and augment the dataset with scale-jittering  \citep{KrizhevskyImageNetNetworks}, or radically change the network architecture \cite{XuScale-InvariantNetwork}, \citep{Han2020ScaleVision}
Even HMAX which was proposed by as a model of position and size invariance object \citep{Riesenhuber1999HierarchicalCortex}, seem to not have a perfect translation or scale invariance \citep{Schneider2002} **HMAX MIGHT BEST BE SKIPPED.  I THINK THEY PUT LIMITED POOLING IN ORDER TO REDUCE INVARIANCE AS THAT IS WHAT THEY CLAIMED THE DATA WERE AT THE TIME. THEY COULD IN PRICIPLE HAVE COMPLETE INVARIANCE I THINK -- ALTHOUGH THE POOLING WOULD PRODUCE SPATIAL INDIFFERENCE AS WELL I EXPECT (Several models have attempted to explain similar phenomena—for instance, HMAX (Serre et al. 2007) pro- vided a conceptual forerunner for our work and evaluated scale- and translation-invariance. Crowding)

VisNet (a non-convolutional model) has also been proposed to account for rotation, translation, and scale invariance \citep{Wallis1997InvariantSystem}

TRANSLATION
If pooling is commonly justified to render the network invariance to change in item scale, the convolution operation is what is supposed to make the network invariant to translation. I THINK POOLING IS OFTEN THOUGHT TO BE KEY FOR TRANSLATION AS WELL.. Though it is commonly assumed that CNN would exhibit a strong tolerance to translation \citep{Gens2014DeepNetworks}, \citep{XuScale-InvariantNetwork} \citep{ConvolutionalNetworks}, most of the studies have actually found very limited translation invariance (\cite{Kauderer-Abrams2017a} \citep{Gong2014Multi-scaleFeatures}, \citep{Azulay2019}, \citep{Chen2017EccentricityVision}, \citep{Blything2020ExtremeTolerance}.
We believe that a deep misunderstanding of this problem is the root of the misconception: the difference between online translation tolerance and trained translation tolerance (\citep{Bowers2016} *FIND RIGHT CITATION IN EXTREME ONLINE ETC.. A network with online tolerance would be able to identify objects at novel locations after being trained on only one location. The degree of tolerance would be defined on how far from the trained location the object can be reliably identified. Trained tolerance, conversely, refers to the identification of a novel examples of an object category, on a location that is already trained on other instances of that category. For instance, a network trained on the whole visual field on identifying instances of dogs, will be able to identify a new image of a dog across multiple locations. This feature is often obtained by data-augmentation: jittering the training images so that the network is trained on example across different locations \citep{Kauderer-Abrams2017a}, \citep{Furukawa2017},  
This can hardly be considered a form of translation invariance. In fact, in this case, the network only needs to generalize to unseen instances of a certain class, on any location. Regardless, these two types of translation tolerance are often confounded together, but they underpin different internal representations. ... 

\section{PREVIOUS WORK}
Very few works have tested the degree of online translation tolerance in CNN. Until recently, most of the reports were unanimously finding no degree of online translation invariance:
\citep{Kauderer-Abrams}, \citep{Chen2017EccentricityVision}}, and \citep{Furukawa2017} tested several CNN architectures (including Resnet-18, but without a global average pooling layer) which invariably showed a very poor online translation tolerance - which could be rescued only by data augmentation. Similarly, \citep{Gong2014Multi-scaleFeatures}  show a significant drop in accuracy followed by horizontal/vertical translation, scaling, rotation, and vertical flipping. 

This failure in tolerance to translation is even more striking when considering that shift-invariance is often used as a motivation for the inclusion of convolution and pooling layers in artificial network \citep{Fukushima1980Neocognitron:Position}\citep{Gens2014DeepNetworks}, \citep{XuScale-InvariantNetwork} \citep{ConvolutionalNetworks},
 Intuitively, when an input is translated, a series of convolution and pooling operators should also result in a simple shift in the activation of the feature map, which would result in being invariant to translation. 
 In practice, \citep{Azulay2019} showed that this is only strictly true when the convolution and pooling networks do not have subsampling (stride of 1) and when these layers are followed by a global average pooling layer.  WERE THESE AUTHORS LOOKING AT ON-LINE OR TRAINED TOLERANCE?  I DON'T THINK STRIDE OF 1 IS NEEDED (OR NEEDED ONLY TO AVOID THE UP AND DOWN PERFORMANCE). These conditions would endow the network with an architectural translation invariance, that is an invariance that is built into the network and does not require any training. In practice, however, these conditions are never satisfied: using a stride of 1 is often computationally unfeasible for image of even discrete size. Plus, the lack of subsampling, and the avoidance of a fully connected layers, may seriously impact the network performace. IS THERE EVIDENCE THAT HAVING MULTPLE LAYERS IMPORTANT IN COME CASES? I WOUDL THINK SO, BUT NOT AWARE... In practice, a lack of architectural TI may not hurt performance much when the network is trained with sufficient data augmentation (fig 11 in Azulay). 

Other 'architectural' solution to the problem of translation have ben suggested: A more general, architectural, solution, that can account to any affine transformation, is provided by the Spatial Transformer Network \citep{Jaderberg2015}; **IS THIS AN ARCHITECTURAL SOLUTION -- OR A WAY TO AUTOMATE DATA AUGMENTATION? invariant-network \citep{Bruna2012InvariantNetworks} \citep{Wallis1997InvariantSystem}.A solution based on Gaussian-Hermite basis to approximate arbitrary filters which would obtain translation invariance has been suggested \citep{Sundaramoorthi}, but it works only on very small shift (up to 1 pixel on x and y direction). It has been suggested that Capsule Net\citep{Sabour2017DynamicCapsules} may actually provde a strong invariance to sever image transformations, however this doesn't seem to be the case Qi Paper 2016 (unpublished). A simple way to endow the network with a sort of architectural translation invariance is to use a global average pooling which would compute the average value of the whole feature map \citep{Blything2020ExtremeTolerance}. This would result in a perfect translation invariance, but would deprive the network to differentiate objects in different spacial locations. WE DON'T HAVE ANY CITATIONS FOR THIS I DON'T THINK.

Without having to resort to new architecture, two works have recently contrasted the previous finding by obtaining a high degree of translation invariance:
\citep{Han2020b} found that a classic CNN (VGG16?) exhibited an almost perfect online translation tolerance on a task with recogniting of Korean characters, but it did not compare these ambiguous results with the previous literature. \citep{Blything2020ExtremeTolerance} firstly found that a perfect online-translation tolerance could be achieved, again with a standard CNN (VGG16, \citep{Symonien}), given that the network was pretrained on ImageNet. \citep{Blything2020ExtremeTolerance}  compared the performance of a ImageNet-pretrained VGG16 and a vanilla one, finding a striking difference in performance on the amount of translation tolerance when the network for then trained on a dataset of 24 3D shapes, the Leek Objects. These results hint to the fact that a translationally invariant representation does not need to be built inside the network architecture, but it can be learn. In the current work, we further explore this idea. \citep{Leek2016EarlyObjects}.

\section{Related Work}
In this work we investigate the extend in which a network can learn implicit properties of its visual environment, specifically the property of translation invariance. 
Why is this important? A network that learns deep characteristic of its visual environment such as being invariant to translation, rotation, etc., is able to accelerate subsequent training in  in that it needs very few training sample for being able to generalize across a wide range of input images. This ability unlocks the skill of 'real' generalization, in which latent visual characteristic can be combined with new training samples. 
Our investigation bears some points in common with other areas os research such as Multi-task learning, Meta-Learning, and learning without forgetting.  Compared to a Multi-task approach, which focuses on learning 'without forgetting' different tasks, we focus on the ability of the network to learn an implicit characteristic of the visual environment, that is a characteristic in which the network is not directly trained upon. Even though we test on multiple recognition tasks, this is used as a way of testing the network ability to retain translation invariance, not because we are directly interested in the network learning multiple tasks. Similarly to Meta-Learning, we want to investigate the ways in which a network can learn how to efficiently learn. But, in this work, instead of focusing on a specific approach, we investigate the cases in which the translation invariance can in fact be extrapolated from the environment. Once that the network has learnt this property, it would be ideal to come up with solution to retain this ability. We see Meta-Learning, Multi-task learning and learning without forgetting as an obvious next step to this work. Instead, here we focus on the more basic problem of the conditions in which such implicit representation can be learnt. 
#



could overcome architectural limitations of the networks. Even though our network is not 'architecturally' invariant nor equivariant (\ref{Int
In Gestalt psychology, one the core principle is that of invariance (citation), amongst which there is the property of the objects to be regarded the same independently of their position in the visual field (invariance to translation). Since birth, humans have perceived a visual environment in which objects were continuously subjected to small translation on their visual field ,through head, eyes movements, etc. This kind of environment, together with the right type of neural-computation mechanism and inductive biases, must have provided the early human brain with the fundamental principle of perceptions. In some sense, the translation invariance, together with other perceptual mechanism employed by the human brain, is embedded into the relationship between the agent and the visual environment in which the agent acts upon.


The fact that ImageNet would provide a network with invariance to translation is, however, purely coincidental, as is it due to the engineering trick of augmenting the dataset, not to desire to provide a network with a naturalisti visual environment. Instead, 


how this would not been needed if artificial networks were trained on naturalistic datasets, more similar to what humans experience in their lifetime, as the characteristic that humans


